Resilient Coordination of Networked Multiagent Systems Based on Distributed State Emulators

This note studies resilient coordination of networked multiagent systems in the presence of misbehaving agents, i.e., agents that are subject to adversaries modeled as exogenous disturbances. Apart from the existing relevant literature that make specific assumptions on the graph topology and/or the fraction of misbehaving agents, we present an adaptive control architecture based on distributed state emulators and show that the nominal networked multiagent system behavior can be retrieved even if all agents are misbehaving.

==> margins.tex <==
\section{Gain Margin Analysis} \label{sec:GM}
Gain margin is an important stability measure originally developed for LTI systems, but the margin can easily be extended to adaptive control. In LTI systems the gain margin is the amount of gain factor that can be added to the feedback loop while maintaining stability. For adaptive systems the gain margin measures the amount of allowable gain between the controlled plant and the adaptive control (\cite{QianSang}).

For our analysis we assume ${\cal{K}}=diag(k_1,k_2,\dots,k_m)$ where $k=k_1=k_2=\dots=k_m > 0$ is the positive gain between the controlled plant and the controller. Notice we assume that the gain is the same for all control channels. Now (\ref{eq:control_law}) becomes $u(t)={\cal{K}}u_{rm}(t)+{\cal{K}}u_{pd}(t)$ and (\ref{eq:edot}) becomes:
\begin{equation}\label{eq:GM_edot}
\dot{e}(t)=A_{rm} e(t) + B{\cal{K}} \tilde{K}^T(t)x(t)+B{\cal{K}} \tilde{K}_r(t)r(t),
\end{equation}
or simply
\begin{equation}\label{eq:GM_edot}
\dot{e}(t)=A_{rm} e(t) + B{k} \tilde{K}^T(t)x(t)+B{k} \tilde{K}_r(t)r(t).
\end{equation}
Consiider the Lyapunov function
\begin{equation} \label{eq:lyap_GM}
V\left(e,\tilde{K},\tilde{K}_r\right)=\frac{1}{2}e^TPe+\frac{1}{2}tr\left(\tilde{K}^T{\bar\Gamma_x}^{-1}\tilde{K}\right)+\frac{1}{2}\tilde{K}^T_r{\bar\Gamma_r}^{-1}\tilde{K}_r.
\end{equation}
where ${\bar\Gamma_x}^{-1}={k}{\Gamma_x}^{-1}$ and ${\bar\Gamma_r}^{-1}={k}{\Gamma_r}^{-1}$.
Differentiating (\ref{eq:lyap_GM}) results:
    \begin{equation}\begin{split}
        \dot V(e(t),\tilde K(t),\tilde {K}_r(t))=&-\frac{1}{2}e^TQe + e^TPB{k}(\tilde K^Tx+ \tilde K_r^T r) \\&- \mathrm{tr}(\tilde{K}^Tk_1(xe^TPB + \sum\limits_{j = 1}^p x_j x^T_j \tilde K)) \\ &- \tilde{K}_r^Tk(re^T PB + \sum\limits_{j = 1}^p r_j r_j \tilde K_r),
    \end{split}\end{equation}
simplfiying:
    \begin{equation}\begin{split}
        \dot V(e(t),\tilde K(t),\tilde {K}_r(t))=&-\frac{1}{2}e^TQe -\mathrm{tr}(\tilde{K}^Tk\sum\limits_{j = 1}^p x_j x^T_j \tilde K) \\ &- \tilde{K}_r^Tk\sum\limits_{j = 1}^p r_j r_j \tilde K_r.
    \end{split}\end{equation}
By following the analysis in \cite{Linear_Chow} the expression can now be reduced to
     \begin{equation}\begin{split}\label{eq:exp_bounds_linear}
        &\dot V(e,\tilde K,\tilde {K}_r)\leq\\&-\frac{\min\left(\lambda_{\min}(Q),2k\lambda_{\min}(\Omega_K),2k\sum\limits_{j = 1}^p r_j^2\right)}{\max\left(\lambda_{\max}(P),\lambda_{\max}(\bar{\Gamma}_x^{-1}),\bar{\Gamma}_r^{-1}\right)}V(e,\tilde K,\tilde {K}_r).
     \end{split}\end{equation}
The system remains exponentially convergent for $k\in(0,+\infty)$.

\section{Time-Delay Margin} \label{sec:TimeDelay}
Unlike the gain margin, the phase margin is not easily extended to adaptive systems. The time-delay margin is the nonlinear analog to phase margin. To our knowledge there are no general methodologies hat have been developed to analyze the time-delay margin of a general adaptive system. Linear approximation techniques have been developed. In this section will be used the findings in \cite{Nguyen_TD} to develop a computable time-delay margin for our adapative system. The main results of the paper will be reviewed first. The first result gives an upper bound on the time-delay margin on a linear system.
\begin{lemma}
Given a time-delay system:
\begin{equation}
\label{eq:delay_system}
\dot{x}(t)=Ax(t)-BKx(t-td)
\end{equation}
where $x(t):[0, \infty) \rightarrow \mathbb{R}^n$ and $A- BK$ is Hurwitz. The time-delay system is asymptotically stable if the following inequalities hold
\begin{eqnarray}\label{eq:timedelay}
t_d<&\frac{1}{\omega}{\cos}^{-1}{\frac{\bar{\mu}(A)+\bar{\mu}(jBK)}{\|BK\|_2}}\\
\omega<&\bar\mu(-jA)+\|BK\|_2
\end{eqnarray}
where
\begin{equation}
\label{eq:mu_functional}
\mu_i(C)=\lambda\left(\frac{C+C^*}{2}\right).
\end{equation}
The proof of this lemma can be found in \cite{Nguyen_TD} and will not be discussed in this paper.
\end{lemma}

	The next result can be used to approximate nonlinear adaptive law without linearization. The comparison lemma approximates the nonlinear adaptive law with a bounded linear version. The lemma is stated as:
\begin{lemma} The equilibrium state of $y(t)=0$ of the differential equation
\begin{equation}
\dot{y}(t)=-{\Phi}^T(t) \Gamma \Phi(t) y(t)
\end{equation}
where $y(t):[0, \infty) \rightarrow \mathbb{R}$,$\Phi(t) \in {\cal{L}}_2 :[0,\infty)\to\mathbb{R}$ is a piecewise continuous and bounded function, and $\Gamma>0\in\mathbb{R}^{n \times n}$, is uniformly asymptotically stable, if there exist a constant $\gamma>0$ such that
\begin{equation}
\frac{1}{T_0}\int_t^{t+T_0}\Phi^T(t)\Gamma\Phi(t)\mathrm{d}\tau\geq\gamma
\end{equation}
which implies that $y(t)$ is locally bounded by the solution of a linear differential equation
\begin{equation}
\dot{z}(t)=-\gamma z(t)
\end{equation}
for $t \in [t_i,t_i+T_0)$, where $t_i=t_{i-1}+T_0$ and $i=1,2,...,n\to\infty$.
\end{lemma}
The proof of the lemma can be founded in \cite{Nguyen_TD} and other sources.

	Now consider a time delay on (\ref{eq:plant_with_control}):
\begin{equation}
\dot{x}(t)=Ax(t)+B(K^T(t-td)x(t-td)+K_r(t-td)r(t-d)),
\end{equation}
and the error expression (\ref{eq:edot}) now becomes:
\begin{equation}\label{eq:edot_td}\begin{split}
\dot{e}(t)=&A_{rm}e(t)+B(K_r(t-td)r(t-td)-K_r^*r(t)\\&+K^T(t-td)x(t-td) -K^*x(t)).
\end{split}\end{equation}
Consider the following expression:
\begin{equation}\label{eq:dotK_linear}\begin{split}
\dot{K}^T(t)x(t)=-B^TPe(t)x^T(t)\Gamma_xx(t)-{\tilde K}^T(t) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x x(t).
\end{split}\end{equation}
Linearization of the second term produces:
\begin{equation}\begin{split}
{\tilde K}^T(t) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x x(t)=&{\tilde K}^T(t_i) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x x(t_i)\\
&+ {\tilde K}^T(t) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x x(t_i) \\
&-{\tilde K}^T(t_i) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x x(t_i) \\
&+ ({\tilde K}^T(t_i)) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x x(t)\\
&- ({\tilde K}^T(t_i)) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x x(t_i)\\
&+ \ldots
\end{split}\end{equation}
and by approximation:
\begin{equation}\begin{split}
{\tilde K}^T(t) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x x(t)\approx&-{\tilde K}^T(t_i) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x x(t_i)\\
&+ {\tilde K}^T(t) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x x(t_i) \\
&+ {\tilde K}^T(t_i) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x x_{rm}(t)\\
&+ {\tilde K}^T(t_i) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x e(t)
\end{split}\end{equation}
for $t\in[t_i,t_i+T_0)$,where $t+0=0,t_i=t_{i-1}+T_0$, and $i=1,2,\dots,n\to\infty$. Returning to (\ref{eq:dotK_linear}) we see that the first term can be approximated with help from lemma 2:
\begin{equation}
-B^TPe(t)x^T(t)\Gamma_xx(t)=-B^TPe(t)\gamma_x
\end{equation}
where $\gamma_x=\inf_{t\in[t_i,t_i+T_0)}\left(\frac{1}{T_0}\int_t^{t+T_0}x^T(t)\Gamma_x x(t)\mathrm{d}\tau\right)\ge0\in\mathbb{R}$. Thus an approximation of (\ref{eq:dotK_linear}) is found. An identical analysis is made for $\dot{K_r}^T(t)r(t)$.
Consider the following:
\begin{equation}\begin{split}
K^T(t)\dot{x}(t)=&K^T(t_i)\dot{x}(t_i)+\dot{K}^T(t_i)\dot{x}(t_i)\Delta t\\&+K^T(t_i)(\dot{x}(t)-\dot{x}(t_i))+\dots
\end{split}\end{equation}
and by approximation:
\begin{equation}
K^T(t)\dot{x}(t)\approx K^T(t_i)\dot{e}(t) + K^T(t_i)\dot{x}_{rm}(t)+\dot{K}^T(t_i)\dot{x}(t_i)\Delta t.
\end{equation}
An identical analysis is made for ${K_r}^T(t)\dot{r}(t)$.
Differentiating (\ref{eq:edot_td}) yields:
\begin{eqnarray*}
\ddot{e}(t)=A_{rm} \dot{e}(t)+B(\dot{K}_rr(t-td)+K_r\dot{r}(t-td)\\
-K_r^*\dot{r}(t)+\dot{K}^T(t-td)x(t-td)\\
+K^T(t-td)\dot{x}(t-td)-K^*\dot{x}(t)).
\end{eqnarray*}
Using the linearization and approximations derived above yields:
\begin{eqnarray*}
\dot{x}(t)
=&
\left[ {\begin{array}{cc}
A_{rm}-B K^{{\star}^T}  & 0 \\
I & 0 \\
\end{array} } \right]
x(t)+\\&
\left[ {\begin{array}{cc}
BK^T(t_i) & -B{\tilde K}^T(t_i) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x-\gamma_{xr} B B^T P \\
0 & 0 \\
\end{array} } \right]
x(t-t_d)\\&
+
\left[ {\begin{array}{cc}
d_1(t-t_d)+d_2 \\
0 \\
\end{array} } \right]
\end{eqnarray*}

where 
$\gamma_{xr}=\gamma_{x}+\gamma_{r}$, $x(t)=
\left[ {\begin{array}{cc}
\dot{e}(t)\\
{e}(t)\\
\end{array} } \right]$,
\begin{equation}\begin{split}
d_2(t-t_d)=&-{\tilde K}_r^T(t-t_d) \sum\limits_{j = 1}^p r_j r^T_j \Gamma_r r(t_i)\\
&-{\tilde K}_r^T(t_i) \sum\limits_{j = 1}^p r_j r^T_j \Gamma_r r(t-t_d)\\
&+ K_r^T(t_i)\dot{r}(t-t_d)-{\tilde K}^T(t-t_d) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_r x(t_i)\\
&-{\tilde K}^T(t_i) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_r x_{rm}(t-t_d)\\
&+K^T(t_i)\dot{x}_{rm}(t-t_d)
\end{split}\end{equation}
\begin{equation}\begin{split}
d_3=& \dot{K}_r^T(t_i)\dot{r}(t_i)\Delta t + {\tilde K}_r^T(t_i) \sum\limits_{j = 1}^p r_j r^T_j \Gamma_r r(t_i)\\
&+ {\tilde K}^T(t_i) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x x(t_i)+\dot{K}^T(t_i)\dot{x}(t_i)\Delta t
\end{split}\end{equation}
are treated as time varying disturbances and do not affect the time-delay margin thus are neglected.

Lemma 2 can be used to determine the time-delay margin of the system:
\begin{eqnarray}
t_{di}<&\frac{1}{\omega}{\cos}^{-1}{\frac{\bar{\mu}(C)+\bar{\mu}(jDK)}{\|DK\|_2}}\\
\omega_i<&\bar\mu(-jC)+\|DK\|_2.
\end{eqnarray}
where
\begin{eqnarray}
C_{i}=&\left[ {\begin{array}{cc}
A_{rm}-BK^{{\star}^T} & 0 \\
I & 0 \\
\end{array} } \right]\\
D_i=&\left[ {\begin{array}{cc}
BK^T(t_i) & -B{\tilde K}^T(t_i) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x-\left(\gamma_{xr}\right) B B^T P \\
0 & 0 \\
\end{array} } \right].
\end{eqnarray}
for for $t\in[t_i,t_i+T_0)$,where $t+0=0,t_i=t_{i-1}+T_0$, and $i=1,2,\dots,n\to\infty$. The time-delay margin is local and is computed for a time window after it has enlapsed.

Another estimation method. We will take $x(t)=
\left[ {\begin{array}{cc}
{e}(t)\\
\tilde{K}^{T}{x}(t)\\
\tilde{K}_r^{T}{x}(t)\\
\end{array} } \right]$, and find a linear estimation for $\dot{x}(t)$. From (\ref{eq:edot_td}) we see that $\dot{x}(t)$ can be written as:
\begin{equation}\begin{split}
\dot{e}(t)=&A_{rm}e(t)+B(\tilde{K}_r(t-td)r(t-td)-K_r^*r(t)\\&+\tilde{K}^T(t-td)x(t-td) -K^*x(t)\\&-{K}^{\star}(t-td)x(t-td)-{K}^{\star}_r(t-td)r(t-td)).
\end{split}\end{equation}
Differentating $\tilde{K}^{T}{x}(t)$ results:
\begin{equation}\begin{split}
\dot{\tilde{K}}^{T}{x}(t)+\tilde{K}^{T}{\dot{x}}(t)=&-B^TPe(t)x^T(t)\Gamma_xx(t)\\&-{\tilde K}^T(t) \sum\limits_{j = 1}^p x_j x^T_j \Gamma_x x(t)\\&+\tilde{K}^{T}(A_{rm}x(t) + B_{rm}r(t)\\& + B \tilde{K}^T(t))x(t)+B \tilde{K}_r(t)r(t),
\end{split}\end{equation}
which can be appromatied by
\begin{equation}\begin{split}
\dot{\tilde{K}}^{T}{x}(t)+\tilde{K}^{T}{\dot{x}}(t)\le&-\gamma_xB^TPe(t)\\&-\lambda_{min}(\sum\limits_{j = 1}^p x_j x^T_j \Gamma_x){\tilde K}^T(t)x(t)\\&+\tilde{K}(t)^{T}(A_{rm}x(t) + B_{rm}r(t))\\& +\tilde{K}(t_i)^{T}( B \tilde{K}^T(t))x(t)+B \tilde{K}_r(t)r(t))).
\end{split}\end{equation}
Differentating $\tilde{K}_r^{T}{r}(t)$ results:
\begin{equation}\begin{split}
\dot{\tilde{K}}_r^{T}{r}(t)+\tilde{K}_r^{T}{\dot{r}}(t)=&-B^TPe(t)r^T(t)\Gamma_r r(t)\\&-{\tilde K}_r^T(t) \sum\limits_{j = 1}^p r_j r^T_j \Gamma_r r(t)\\&+\tilde{K}_r^{T}{\dot{r}}(t),
\end{split}\end{equation}
which can be appromatied by
\begin{equation}\begin{split}
\dot{\tilde{K}}_r^{T}{r}(t)+\tilde{K}_r^{T}{\dot{r}}(t)\le&-\gamma_rB^TPe(t)\\&-\lambda_{min}(\sum\limits_{j = 1}^p r_j r^T_j \Gamma_r){\tilde K}_r^T(t)x(t)\\&+\tilde{K}_r^{T}{\dot{r}}(t).
\end{split}\end{equation}
We can then estimate the adaptive system as a LTI system in a given time window,
\begin{eqnarray*}
\dot{x}(t)
\le &
\left[ {\begin{array}{ccc}
A_{rm} & 0  & 0 \\
-\gamma_x B^{T} P & \tilde{K}^{T}(t_i) B-\lambda_{min}(\sum\limits_{j = 1}^p x_j x^T_j \Gamma_x) & \tilde{K}^{T}(t_i) B  \\
-\gamma_r B^{T} P & 0 & -\lambda_{min}(\sum\limits_{j = 1}^p r_j r^T_j \Gamma_r)\\
\end{array} } \right]
x(t)\\&+
\left[ {\begin{array}{ccc}
0& B & B \\
0 & 0 & 0 \\
0 & 0 & 0 \\
\end{array} } \right]
x(t-t_d)\\&
+
\left[ {\begin{array}{c}
-B(K^{\star}x(t)+K_r^{\star}r(t)+K(t-t_d)x(t-t_d)+K_r(t-t_d)r(t-t_d)\\
\tilde{K}^{T}(A_{rm}x(t)+B_{rm}r(t)) \\
\tilde{K}^{T}_r \dot{r}(t)\\
\end{array} } \right]
\end{eqnarray*}
